Entertain, then Cancel: How Thinking Makes Reasoning Models Read Some and Or Literally

When a speaker says ``some students passed'', listeners infer that not all of them did. Reasoning models now let users decide how long a model thinks before it answers, but we do not know what extra thinking does to such everyday inferences. We study this directly: we keep a model's weights fixed, change only how much it thinks, and record which reading it chooses. A second tool cuts the model's own reasoning at successive points and asks for an answer, showing where the reading changes. Thinking makes models read logical words as logic: it cancels the implicatures of \emph{some} (\emph{not all}) and \emph{or} (\emph{not both}) in most tested open reasoning models and in GPT-5, while context-driven inferences such as indirect answers improve. The trace shows why: models first entertain the enriched reading and cancel it later. Answering from that early reading, an exploratory inference-time remedy, recovers these implicatures without losing literal accuracy. Evaluations of reasoning models should measure how they interpret, not only how accurate they are.

==> sections/5_origin.tex <==
\section{Where the Literal Default Comes From, and How an Intent Seed Shifts It}
\label{sec:origin}

% Best-paper pass (2026-10-04). Details and the full method comparison: App. app:results.

\subsection{Post-Training Moves the Default Reading}
\label{sec:origin:stages}

\input{tables/tab_ist}

If thinking cancels a default, training for thinking may also move the default itself. We score every stage of three lineages without deliberation, from the log-probabilities of the two answers, and measure the cost of thinking within each stage that can think (\Cref{tab:stages}).
Post-training for reasoning moves the default reading of \form{some} towards the literal one, at a stage that depends on the recipe.
In OLMo-3, the pragmatic default falls from \res{e2.olmo3-7b-base.a3-quant.inf.lp4.R.mean}\% in the base model to \res{e2.olmo3-think-sft.a3-quant.inf.lp4.R.mean}\% after supervised fine-tuning on thinking traces, whereas reinforcement learning on math from the same base (RL-Zero) leaves it at \res{e2.olmo3-rlzero-math-final.a3-quant.inf.lp4.R.mean}\%.
In Tülu-3 the change comes with preference tuning (DPO), from \res{e2.tulu3-8b-sft.a3-quant.inf.lp4.R.mean}\% to \res{e2.tulu3-8b-dpo.a3-quant.inf.lp4.R.mean}\%, and the following reinforcement learning from verifiable rewards (\rlvr) leaves it there.
As the default turns literal, the extra cost of thinking shrinks: within OLMo-3-Think the cost of thinking on \form{some} shrinks from \res{e2t.olmo3-think-dpo.a3-quant.inf.nat.dR.mean}\,pp at the preference-tuning stage to \res{e2t.olmo3-think-s1375.a3-quant.inf.nat.dR.mean}\,pp after the final RL step.
Distillation from reasoning traces does not have this effect in every lineage: R1-Distill-Qwen-7B reads \form{some} pragmatically in \res{e2.r1distill-qwen-7b.a3-quant.inf.lp4.R.mean}\% of items, against \res{e2.qwen25-7b.a3-quant.inf.lp4.R.mean}\% for its base model.

\noindent\textbf{Takeaway: the literal default of logical words emerges during post-training, at a recipe-dependent stage (thinking SFT in OLMo-3, preference tuning in Tülu-3), and not in the RL-Zero and distillation comparisons we tested.}

\subsection{One Sentence of Speaker Intent Restores Part of the Enrichment}
\label{sec:origin:ist}

If the literal reading comes from what thinking is spent on, the start of the trace should matter. \emph{Intent-Seeded Thinking} (\method) opens the thinking block with one fixed sentence about what the speaker intends to convey; two control sentences of the same length (26 tokens) ask for careful step-by-step reasoning or for checking what the words strictly entail (\Cref{app:method}).
The intent seed yields the most enrichment of the three seeds (\Cref{tab:ist}). In Qwen3-8B it raises the pragmatic reading of \form{some} from \res{e10.qwen3-8b.a3-quant.inf.nat.R.mean}\% under natural thinking to \res{e10.qwen3-8b.a3-quant.inf.sint.R.mean}\% (\res{e10.qwen3-8b.a3-quant.inf.off.R.mean}\% without thinking), against \res{e10.qwen3-8b.a3-quant.inf.sneu.R.mean}\% with the neutral seed; in Qwen3-32B it raises it from \res{e10.qwen3-32b.a3-quant.inf.nat.R.mean}\% to \res{e10.qwen3-32b.a3-quant.inf.sint.R.mean}\%, while both controls leave it at or below the natural level there. Accuracy on indirect answers moves from \res{e10.qwen3-8b.b2.yn.nat.acc.mean}\% to \res{e10.qwen3-8b.b2.yn.sint.acc.mean}\%.
On the newest generation the seed lifts the reading above its no-thinking level: Qwen3.5-9B reads \form{some} pragmatically in \res{e10.qwen3p5-9b.a3-quant.inf.sint.R.mean}\% of items with the seed, against \res{e10.qwen3p5-9b.a3-quant.inf.nat.R.mean}\% under natural thinking and \res{e10.qwen3p5-9b.a3-quant.inf.off.R.mean}\% without thinking, while the neutral and logic seeds reach \res{e10.qwen3p5-9b.a3-quant.inf.sneu.R.mean}\% and \res{e10.qwen3p5-9b.a3-quant.inf.slog.R.mean}\%.
Prompted chain-of-thought with thinking off moves the reading less than native thinking does, so producing a chain of thought is not enough to cause the full shift.

\noindent\textbf{Takeaway: what the trace starts with steers the reading chosen; a sentence about speaker intent recovers more of the lost enrichment than length-matched control sentences.}


==> sections/5_remedies.tex <==
\section{Four Pre-Registered Remedies Fail}
\label{sec:remedies}

If thinking cancels an enrichment it first entertains, a remedy should keep the entertained reading where the context licenses it. We pre-registered four remedies on Qwen3-8B, each with a matched control and safety gates (one-sided 95\% bounds above $-2$\,pp on ImplicatureX cancellation, IMPPRES true/false framing, FOLIO and GSM8K), and applied a fixed one-shot rule: a remedy reaches the held-out test set only if it beats natural thinking and passes every gate on development items. \Cref{tab:remedies} shows that none does.
Prompting backfires: a check before thinking ends, asking whether the question concerns entailment or the speaker's meaning, lowers speaker-meaning accuracy from \res{m1dev.qwen3-8b.v2.nat.speaker.mean}\% to \res{m1dev.qwen3-8b.v2.sitcheck.speaker.mean}\%, turning \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.r2w.mean} correct answers wrong, while a neutral check of the same length leaves it at \res{m1dev.qwen3-8b.v2.neutral.speaker.mean}\%; raising the entailment question is enough to trigger the cancellation. Training does not beat its controls: fine-tuning on the model's own correct, family-balanced traces matches fine-tuning on unselected ones, and preference optimisation on correct-versus-incorrect pairs edges past shuffled pairs without passing the gates. Two exploratory inference-time remedies built on the entertained reading, frozen before running, change no development answer under their input-only routing, and with larger weights every answer they change gets worse (\Cref{tab:xgrid}). Designs, controls and per-set results are in \Cref{app:remedies}.
\input{tables/tab_remedies}


==> sections/5_sit.tex <==
\section{Speaker-Intent Tuning Trains Task-Appropriate Interpretation}
\label{sec:sit}

% METHOD (notes/METHOD_DESIGN.md: v1 seeds and v2 late check failed their pre-declared dev gates; SIT = D-contingency, pre-declared 2026-10-05).

Because early trace prefixes elicit enriched answers that typically vanish by completion, we tested whether a prompt in the thinking channel could preserve them. Both tested interventions, however, fail their pre-declared safety gates on Qwen3-8B development items.

\paragraph{Both tested thinking-channel prompts fail the safety gates.}
On development items for Qwen3-8B, we tested training-free interventions against pre-declared safety gates (\Cref{app:m1dev}).
\begin{itemize}[nosep,leftmargin=*]
  \item \emph{Opening the trace with a sentence about speaker intent} lowers both families. With the route wording, speaker-meaning accuracy falls from \res{m1dev.qwen3-8b.v1.nat.speaker.mean}\% to \res{m1dev.qwen3-8b.v1.route.speaker.mean}\% and literal accuracy from \res{m1dev.qwen3-8b.v1.nat.literal.mean}\% to \res{m1dev.qwen3-8b.v1.route.literal.mean}\%.
  \item \emph{A task-sensitive check before the thinking block closes} (``does the question ask what the words strictly entail, or what the speaker means?'') makes the model more literal still. Speaker-meaning accuracy falls from \res{m1dev.qwen3-8b.v2.nat.speaker.mean}\% to \res{m1dev.qwen3-8b.v2.sitcheck.speaker.mean}\% (\res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.r2w.mean} answers turn wrong, \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.w2r.mean} turn right). A neutral check of the same length leaves it at \res{m1dev.qwen3-8b.v2.neutral.speaker.mean}\%.
\end{itemize}
The task-sensitive check degrades speaker-meaning accuracy more than the same-length neutral check, implicating the prompt's content rather than mere repetition. This motivates training task-appropriate interpretations instead of relying on prompting.

\paragraph{Speaker-Intent Tuning.}
\emph{Speaker-Intent Tuning} (\sit) fine-tunes a model on its own natural-thinking traces, selected so that interpretation is rewarded rather than enrichment.
\begin{itemize}[nosep,leftmargin=*]
  \item \emph{Sampling.} For each training item we sample four traces and keep at most one whose answer matches the original gold label.
  \item \emph{Balance.} Each family gets the same number of traces: speaker meaning, presupposition, and literal-gold items, including logic and arithmetic. The selected traces supervise enriching where the context licenses it and staying literal where the task asks for entailment.
  \item \emph{Difficulty.} Items that the model answers correctly only sometimes fill the quota first, so the signal comes from items where its reading varies.
\end{itemize}
We train LoRA adapters (rank 16; two epochs; settings fixed in advance, final checkpoint only) on Qwen3-8B and on DeepSeek-R1-0528-Qwen3-8B, which shares the base model but has different post-training. The training items come from template families disjoint from both development and test.

\paragraph{Preference variant.} As a fourth and final pre-registered attempt, \sit-DPO trains on pairs of a correct and an incorrect trace for the same item (direct preference optimisation, LoRA, settings fixed in advance), against a control with the pair labels shuffled.


==> sections/6_sit_results.tex <==
\section{Experiments}
\label{sec:sit:results}

\subsection{Experimental Settings}
\label{sec:sit:settings}
\textbf{Datasets.} Development items cover the three families of \Cref{sec:sit}; test template families are held out and, because no variant qualified, were never used for any remedy.

\textbf{Baselines.} Each trained variant has a matched control: supervised fine-tuning on the same number of unselected traces, and preference optimisation on the same pairs with shuffled labels. Training-free arms are natural thinking, no thinking, a 512-token budget, a task-aware instruction and the two thinking-channel checks.

\textbf{Metrics.} A variant qualifies for the test set only if it beats natural thinking on the equal-family score and passes one-sided 95\% safety bounds above $-2$\,pp on ImplicatureX cancellation, the true/false framing of the IMPPRES items, FOLIO \citep{han2024folio} and GSM8K \citep{cobbe2021gsm8k}.

\subsection{Main Results}
\label{sec:sit:main}
\Cref{tab:dqual} reports the development results of the trained variants. No variant passes the safety gates, and supervised fine-tuning does not beat its own control. In Qwen3-8B, fine-tuning on selected traces scores \res{m1dev.qwen3-8b.d.sit.score.mean}, the same amount of unselected traces \res{m1dev.qwen3-8b.d.control.score.mean}, and natural thinking \res{m1dev.qwen3-8b.d.nat.score.mean}; in DeepSeek-R1-0528-Qwen3-8B the three score \res{m1dev.r1-0528.d.sit.score.mean}, \res{m1dev.r1-0528.d.control.score.mean} and \res{m1dev.r1-0528.d.nat.score.mean}. Tuning shortens the thinking of DeepSeek-R1-0528-Qwen3-8B from \res{m1dev.r1-0528.d.nat.tokfc.mean} to \res{m1dev.r1-0528.d.sit.tokfc.mean} tokens per item, but the unselected control does so as well (\res{m1dev.r1-0528.d.control.tokfc.mean}). Preference optimisation on correct-versus-incorrect pairs edges past its shuffled control, \res{m1dev.qwen3-8b.e.dpo.score.mean} against \res{m1dev.qwen3-8b.e.dposhuf.score.mean} in Qwen3-8B and \res{m1dev.r1-0528.e.dpo.score.mean} against \res{m1dev.r1-0528.e.dposhuf.score.mean} in DeepSeek-R1-0528-Qwen3-8B, where speaker-meaning accuracy rises from \res{m1dev.r1-0528.e.nat.speaker.mean}\% to \res{m1dev.r1-0528.e.dpo.speaker.mean}\%; it still misses the safety gates, so no remedy reached the test set.
\input{tables/tab_dqual}

\textbf{Prompting the thinking backfires.} The task-sensitive late check turns \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.r2w.mean} correct speaker-meaning answers of Qwen3-8B wrong and only \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.w2r.mean} wrong answers right; a neutral check of the same length leaves accuracy at \res{m1dev.qwen3-8b.v2.neutral.speaker.mean}\%. Raising the entailment question is enough to trigger the literal reading that thinking produces on its own.

\subsection{Ablation Study}
\label{sec:sit:ablation}
\Cref{tab:ablation} removes one component of \sit at a time on the development items of Qwen3-8B. No training-free intervention passes all safety gates: the late check costs \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.r2w.mean} correct speaker-meaning answers, the start-of-thinking seed lowers both families, and even the best training-free arm, the task-aware instruction, misses a gate. Trained on its own traces, the model changes little, and neither component of \sit matters: the full model scores \res{m1dev.qwen3-8b.v3.sit.score.mean}, w/o trace selection \res{m1dev.qwen3-8b.v3.control.score.mean} and w/o family balance \res{m1dev.qwen3-8b.v3.nobal.score.mean}, against \res{m1dev.qwen3-8b.v3.nat.score.mean} for natural thinking.
\input{tables/tab_ablation}


==> sections/A1_related.tex <==
\FloatBarrier
\section{Background}
\label{app:g-bg}
This part reviews related work and states the theoretical accounts and pre-registered hypotheses.

\FloatBarrier
\subsection{Related Work}
\label{sec:related}\label{app:related}
This section reviews related work on implicature, reasoning models and test-time compute.


% Closest work first; each paragraph closes with the contrast (STYLE_GUIDE 3.6).
% Positioning table and verification log: notes/RELATED_WORK.md.

\paragraph{Test-time reasoning and social understanding.}
Several studies find that reasoning does not transfer to social cognition.
Reasoning variants of Qwen3 and DeepSeek do no better than their non-reasoning counterparts on theory-of-mind benchmarks, and o3's accuracy on higher-order belief questions falls as reasoning effort rises \citep{gong2026think}. Reasoning models also trail older models on theory-of-mind variants of cognitive-science experiments \citep{lupu2025decrypto}, and the gains they do show are better described as robustness to prompt variation than as new ability \citep{dehaan2026reasoning,dehaan2026evaluating}.
For presupposition, models with stronger reasoning give less human-like projection judgements \citep{azin-etal-2026-presupposition}, and reasoning adds only 2--11 points on queries with false presuppositions \citep{sathyanathan-etal-2026-evaluating}.
On implicature the record is mixed.
The closest observation is incidental: in ImplicatureX, a benchmark of implicature recognition and cancellation, Qwen3 in thinking mode at a 512-token budget recognises fewer scalar implicatures than the same weights without thinking, and recognises cancellations more often \citep{spinoso2026evaluating}.
Chain-of-thought (CoT) prompts built on Grice's maxims, on relevance theory or on the Rational Speech Act model improve implicature resolution and number-word interpretation \citep{kim2023pope,sato2025pragmatic,tsvilodub2025nonliteral}; CoT lifts GPT-4 to human average on binary implicatures \citep{ruis2023goldilocks}; and training on counterfactual reasoning traces helps further \citep{park2026pragrest,sravanthi-etal-2025-understand}. Yet CoT was also observed to ``encourage literal interpretations'' in Korean \citep{park-etal-2024-pragmatic}.
% Closing contrast: verbatim anchor from notes/PAPER_OUTLINE.md v1.1 (design reviewer, REVIEW_design_fable.md sec. H).
% RESULTS-DEPENDENT: "show", "locate", "remove" must be re-checked against the results at the Oct 3 gate.
Unlike ImplicatureX, which observes the drop at a single budget on 46 items without intervals and does not treat it as a thinking effect, and unlike \citet{gong2026think}, who study the same manipulations on theory-of-mind accuracy, we treat the thinking budget as a controlled dose, measure the reading chosen under felicity and truth framings, show that the effect dissociates by implicature type, trace it to an entertain-then-cancel trajectory inside the trace and to specific post-training stages (thinking SFT in OLMo-3, preference tuning in Tülu-3), and test four pre-registered remedies under matched controls.

\paragraph{Pragmatics in language models.}
Benchmarks cover implicature, indirect speech, irony, metaphor, humour, deceit and presupposition \citep{hu-etal-2023-fine,ruis2023goldilocks,sravanthi-etal-2024-pub,jeretic-etal-2020-natural,liu-etal-2022-testing}; see \citet{ma-etal-2025-pragmatics} for a survey.
When models err on these items, their errors favour the literal reading over distractors \citep{hu-etal-2023-fine}.
Work on scalar implicature links model expectations over alternatives to human inference rates \citep{schuster-etal-2020-harnessing,hu-etal-2023-expectations}, probes scalar diversity \citep{lin-etal-2024-probing}, and steers graded interpretations through activations \citep{cho2026continuous}. Thinking and instruct models have also been compared on quantifier production, across models \citep{montero2025quantification}.
Pragmatic competence rises from base to SFT and preference-tuned checkpoints \citep{yu-etal-2026-pragmatic}. This is why comparisons across training stages confound deliberation with post-training.
Unlike these works, we treat the inference budget as the independent variable, hold the weights fixed for the primary contrast, and extend the stage analysis from supervised fine-tuning through preference tuning to \rlvr.

\paragraph{Overthinking and side effects of reasoning training.}
Longer reasoning can lower accuracy on easy problems, on tasks with distractors and on deduction \citep{chen2024overthinking,gema2025inverse,ghosal2025thinking,lee2026lost,sui2025stop}. Explicit reasoning also degrades instruction following \citep{li2025thinking}, and CoT hurts where deliberation hurts humans \citep{liu2024mind}, while its benefits concentrate on math and symbolic tasks \citep{sprague2025cot}.
Reinforcement fine-tuning has side effects of its own: it lowers refusals on unanswerable questions \citep{song2025hallucination}, can raise hallucination \citep{yao2025hallucination}, and may sharpen what the base model already does rather than extend it \citep{yue2025does}.
Budget forcing \citep{muennighoff-etal-2025-s1}, hybrid thinking modes \citep{yang2025qwen3} and effort levels \citep{openai2025gptoss} make the amount of reasoning controllable; recent work also asks how reasoning changes social behaviours such as sycophancy \citep{feng-etal-2026-good}.
These works define harm as lower accuracy on tasks with one correct answer.
Our outcome is a choice between two readings that are both licensed by the sentence. The direction of the shift, not its size, is what distinguishes the two theories.

\paragraph{The processing cost of enrichment in humans.}
Human evidence that scalar enrichment is effortful comes from response times, deadlines and dual-task load \citep{bott2004some,deneys2007logical,dieussaert2011some,marty2013scalar,tomlinson2013possibly}, and from development \citep{noveck2001children}. Counter-evidence shows that the cost depends on context and on the availability of alternatives \citep{breheny2006generalised,grodner2010some,degen2015processing}.
Enrichment rates also vary widely across scales \citep{vantiel2016scalar,gotzner2018scalar,pankratz2021role}, and probabilistic models treat enrichment as inference about a cooperative speaker \citep{frank2012predicting,goodman2016pragmatic,goodman2013knowledge}.
We import the manipulation from this literature (a controlled change in deliberation), not its conclusion. \Cref{app:theory} derives what each account predicts for a model.


==> sections/A2_theory.tex <==
\FloatBarrier
\subsection{Accounts, Hypotheses and Operationalisation}
\label{sec:theory}\label{app:theory}
This section states the theoretical accounts, the pre-registered hypotheses and how each is operationalised.


% Theory -> thesis -> operationalisation -> hypotheses. Story-neutral v0 (2026-09-30):
% notes/STORIES.md pre-registers Story A (uniform default-and-cancel) and Story B
% (capability-dependent crossover); the decision rule is in STORIES.md and plan sec. 2.
% Title alternatives: A "Two Accounts of What Enrichment Costs";
%                     B "Enrichment Emerges with Capability, as It Does in Children".

\paragraph{Generalized and particularized implicatures.}
\citet{grice1975logic} distinguished \emph{generalized conversational implicatures}, which an expression carries unless the context blocks them (\form{some} conveys \gloss{not all}), from \emph{particularized conversational implicatures}, which arise only from a specific context (``I wore gloves'' in answer to ``Did you leave fingerprints?'' conveys \gloss{no}). We call them \gcis and \pcis.
The two major post-Gricean theories disagree about \gcis. On the \emph{default} view \citep{levinson2000presumptive}, a \gci is generated automatically and cancelled only when the context contradicts it. On the relevance-theoretic view \citep{sperber1986relevance}, every implicature is an inference drawn when it pays off in relevance, and drawing it costs processing effort. Both treat \pcis as context-driven inferences.

\paragraph{Adults pay for enrichment; children often do not make it.}
Adults who reject an underinformative sentence such as ``Some elephants are mammals'' take longer than adults who accept it, and a short response deadline yields fewer rejections \citep{bott2004some}. A concurrent memory load does the same \citep{deneys2007logical,dieussaert2011some,marty2013scalar}.
The finding is contested. Scalar inferences depend on context \citep{breheny2006generalised,degen2015investigating} and can be immediate when the alternatives are salient \citep{grodner2010some,degen2015processing}, although other studies find a delay \citep{huang2009online}.
Development adds a second axis. Children accept underinformative \form{some} far more often than adults do \citep{noveck2001children,papafragou2003scalar}. Yet the same children give such sentences the middle value on a three-point scale, so they notice the violation and tolerate it \citep{katsos2011pragmatic}. On this view, enrichment grows with the listener's resources and competence, and the ``logician'' is a developmental stage, not a default.
For \pcis the human record differs again. Conventional indirect requests are understood without first computing their literal meaning \citep{gibbs1983literal}, and salient figurative meanings can be accessed directly \citep{giora1997understanding}.

\paragraph{Test-time thinking as a dose of deliberation.}
A reasoning model with a thinking toggle and a budget exposes what no human experiment can: the same weights answering the same item with more or less deliberation.
We use \emph{default} operationally, as the reading a model chooses at zero deliberation, and \emph{cancel} for a change of that reading towards the literal one as deliberation is added; neither term presupposes a cognitive mechanism.
We consider three profiles.
\begin{itemize}
  \item On the \emph{effort account}, enrichment is effortful, and more thinking yields more pragmatic readings on every phenomenon we test.
  \item On the \emph{default-and-cancel account}, the model holds \gcis as defaults and spends deliberation on truth-conditional verification, a habit that training with verifiable rewards (\rlvr) plausibly rewards. Thinking then \emph{cancels} \gcis while it improves \pcis, whose pragmatic reading can only be reached by inference.
  \item On the \emph{capability account}, deliberation amplifies whichever competence dominates the trace, so the sign of the effect on \gcis depends on the model's capability, much as enrichment depends on age in children.
\end{itemize}
The theory question is therefore:
\begin{center}
\emph{Do reasoning models pay the cost of enrichment, or the cost of cancelling it, and does that depend on capability?}
\end{center}

\begin{claimbox}
Test-time thinking is a dose of deliberation on fixed weights. If pragmatic enrichment in language models is effortful, more thinking yields more enrichment on every phenomenon; if training with verifiable rewards installs a default-and-cancel profile, thinking cancels generalized implicatures while it improves particularized ones; if deliberation amplifies existing competence, the sign on generalized implicatures reverses with capability.
\end{claimbox}

\paragraph{Operationalisation.}
The dependent variable is the \emph{reading chosen}: $\rate$ is the proportion of committed answers that take the pragmatic reading. For \pcis the pragmatic reading is the correct answer, so $\rate$ is accuracy.
The dose is the \emph{thinking budget} $B$, from no thinking (\NT) through capped budgets to natural stopping under an 8{,}192-token safety cap (\NAT). Its log, $x=\log_2(B+1)$, enters the statistical models.
Under a true/false instruction, the literal answer to ``Some elephants are mammals'' is \emph{correct}. A model that reads the question as a logic problem would therefore drift literal with thinking for reasons that have nothing to do with enrichment; we call this \emph{logic-mode compliance}. The primary readouts are judgements of felicity rather than truth, and the true/false framing serves as the logic-mode comparison.
Binary judgements also hide pragmatic tolerance. Category sentences are therefore judged on a ternary scale (completely right / a bit wrong / completely wrong; both lower values count as pragmatic) and on a 1--7 scale \citep{katsos2011pragmatic,degen2015investigating}, with binary felicity and truth judgements as comparisons.
Binary judgements of category sentences stay near the literal ceiling (\res{e1.qwen3-8b.a1.fel.off.lit.mean}\% literal for Qwen3-8B without thinking), whereas a majority of adults reject such sentences (54--100\% across tasks; \citealp{deneys2007logical,marty2013scalar,katsos2011pragmatic}).
\Cref{tab:operationalization} maps each prediction to its measurement.

\input{tables/tab_operationalization}

\paragraph{Hypotheses.}
Hypotheses, thresholds, falsifiers and the rule that decides between the three profiles were fixed before the main runs (\Cref{app:stats}).

\begin{hypothesis}[Direction on \gcis]\label{hyp:direction}
Under the felicity framings, the effort account predicts that $\rate$ on \gcis rises with $x$; the default-and-cancel account predicts that it falls. A direction counts if $|\Delta\rate|$ between \NT and \NAT is at least 5\,pp with non-overlapping 95\% confidence intervals, with the same sign under capped and length-stratified budgets and under both readouts. Default-and-cancel predicts the shift under both framings, whereas logic-mode compliance predicts it under true/false only. \emph{Falsified} for both accounts if $\Delta\rate$ is equivalent to zero within $\pm3$\,pp at every size.
(\hyp{1b}, capability) The capability account predicts that $\Delta\rate$ is negative for the smallest models and positive for at least one model of 32B or more, that its sign is ordered by a capability measure rather than by training recipe, and that the flip reproduces within a same-recipe size pair.
\end{hypothesis}

\begin{hypothesis}[Split]\label{hyp:split}
Thinking raises accuracy and lowers the literal-error share on \pcis while it lowers $\rate$ on \gcis, a budget $\times$ class interaction. The claim is about the class average, with a random effect for item set. It holds if the interaction is significant and at least three \pci sets improve or stay flat under natural thinking; a drop confined to a capped budget counts as a truncation cost. \emph{Falsified} if \gcis and \pcis move in the same direction, or if \pci accuracy drops under natural thinking on at least half of the sets.
Two corollaries follow.
(\hyp{2b}) A pragmatic listener enriches more when the speaker has full knowledge \citep{goodman2013knowledge}. Default-and-cancel predicts that thinking lowers $\rate$ in both knowledge conditions; the effort and capability accounts predict that thinking widens the gap between them.
(\hyp{2c}) Asking whether an implicated interpretation is \emph{true} should make thinking deny it for \gcis and \pcis alike, as in the one prior same-weights contrast (\citealp{spinoso2026evaluating}, Tables~6--7). Asking what the speaker \emph{meant} should instead let \pcis improve. \emph{Falsified} if \pci accuracy under the meaning framing also drops, or if the truth-framing drop is absent for \pcis.
\end{hypothesis}

\begin{hypothesis}[Training origin]\label{hyp:origin}
The literal shift is installed by \rlvr. We test two estimands. \emph{H3-default}: the default reading, scored without deliberation, turns literal at the \rlvr stage and, in zero-RL runs, with RL steps. \emph{H3-cost}: the within-stage cost of thinking appears or grows at the \rlvr stage. \emph{Falsified} if the change appears at SFT, if at most two of five RL-Zero series trend, or if distilled thinkers show the same cost as RL-trained ones.
\end{hypothesis}

\begin{hypothesis}[Load]\label{hyp:load}
A memory load lowers $\rate$ on \gcis without thinking, as in humans. The load $\times$ thinking interaction shows whether thinking acts as a resource or as the canceller. \emph{Falsified} if load moves $\rate$ by less than 3\,pp at both thinking levels.
\end{hypothesis}

\begin{hypothesis}[Human ordering]\label{hyp:human}
At the smallest budget, literal rates per scale correlate with human rates (Spearman $\rho \geq 0.3$, with a CI excluding 0).
\end{hypothesis}

\begin{hypothesis}[Restorable]\label{hyp:restore}
One fixed sentence about speaker intent, placed inside the thinking channel (\emph{Intent-Seeded Thinking}, \method), restores at least half of a negative \gci shift, with \pci accuracy non-inferior within 1\,pp. \emph{Falsified} if a token-matched neutral sentence restores as much.
\end{hypothesis}

\begin{hypothesis}[Locus]\label{hyp:locus}
Read at successive prefixes of a trace, the answer-position preference starts near its no-thinking value and crosses to the literal reading inside the trace, after literalness markers such as \form{technically} and \form{strictly speaking}.
\end{hypothesis}


==> sections/A3_method_details.tex <==
\FloatBarrier
\section{Experimental Setup}
\label{app:g-setup}
This part gives the items, models, decoding, auditing and prior-work baselines.

\FloatBarrier
\subsection{Method Details}
\label{app:method}
This section gives the item sets, readouts, data splits and statistical tests in full.


% Moved from the main-text method section in the Oct 4 best-paper pass; the main text keeps the core definitions (Sec. 3).
\paragraph{Models and checkpoints.}
The primary manipulation needs a model whose thinking can be switched and dosed without changing its weights. Qwen3 has a hybrid thinking mode in which the no-thinking template differs from the thinking template only by an empty thinking block \citep{yang2025qwen3}. We therefore use Qwen3-4B, 8B and 14B as the primary models, and 1.7B and 32B for size.
The Qwen3 size ladder is also a training-recipe ladder: the 0.6B--14B models are built by strong-to-weak distillation from larger models, whereas the 32B and 235B models go through the full four-stage pipeline with reasoning and general RL (\citealp{yang2025qwen3}, §4.5). Size and recipe are therefore confounded within Qwen3, and we separate them with two same-recipe size pairs, OLMo-3-7B-Think vs.\ OLMo-3-32B-Think and gpt-oss-20b vs.\ 120b. As a capability covariate we use each model's accuracy on a fixed subset of MATH-500 without thinking.
gpt-oss-20b and 120b add a second family with three reasoning-effort levels \citep{openai2025gptoss}. We use them only if the realised reasoning length grows monotonically with the level on held-out items.
To locate the training origin, we score checkpoints along base $\rightarrow$ SFT $\rightarrow$ DPO $\rightarrow$ \rlvr lineages: OLMo-2 \citep{olmo2025olmo2}, OLMo-3-Think \citep{olmo2025olmo3} and Tülu-3 from SFT onward \citep{lambert2024tulu}.
We also score the OLMo-3 RL-Zero series, which applies \rlvr to one base model in five reward domains (math, code, instruction following, general, mixed), at six log-spaced steps each.
Distilled thinkers \citep{deepseekai2025r1} and zero-RL pairs \citep{zeng2025simplerl,hu2025openreasonerzero} are a secondary contrast, because their weights differ from their bases in more than training stage \citep{yu-etal-2026-pragmatic}.
All models are open weights and ungated. \Cref{app:models} lists identifiers and revisions.

\paragraph{Data.}
Items fall into three classes. \emph{Generalized implicatures} (\gcis) comprise Bott--Noveck-style category sentences written for this study (six sentence types per category triple, every item screened by two Claude-family LLM raters and an open-weight co-rater (Qwen3-32B) on the same items, with disagreements dropped the Qwen3-32B co-rater pass is in \texttt{exp/gold/item\_screen\_qwen32b.jsonl}; \Cref{app:details}); scalar-diversity sentences with human inference rates per scale \citep{vantiel2016scalar,gotzner2018scalar,pankratz2021role,hu-etal-2023-expectations}; and IMPPRES implicature pairs whose logical and pragmatic labels differ, plus fresh paraphrased minimal pairs \citep{jeretic-etal-2020-natural}.
\emph{Particularized implicatures} (\pcis) come from PragMega \citep{hu-etal-2023-fine}, LUDWIG \citep{ruis2023goldilocks}, Fig-QA \citep{liu-etal-2022-testing} and six PUB tasks \citep{sravanthi-etal-2024-pub}.
\emph{Presupposition} items come from IMPPRES.
We also run all of ImplicatureX as a replication set \citep{spinoso2026evaluating}.
Released sets that predate the thinking models may be contaminated. We therefore report headline \gci numbers on the fresh items and treat released sets as replications; the within-item contrast between thinking conditions does not depend on whether an item was seen in training.
Items are split 50/50 into development and test halves, stratified by set. Every finding is reported on the test half.
 Sources, licences and item counts are listed in \Cref{app:details}.

\paragraph{Framings.}
Scalar items are asked two ways. \emph{Felicity} framings make the literal answer a pragmatic failure and are primary. For IMPPRES this is an inference question (``Would you conclude that the speaker believes \ldots?''). For the category sentences it is a ternary judgement (completely right / a bit wrong / completely wrong) and a 1--7 rating, with binary felicity (``Is this a good way to describe the facts?'') as a comparison. The \emph{truth} framing (``Is the sentence true or false?'') is the logic-mode comparison (\Cref{sec:theory}).
\pci items use their native meaning format (``What did the speaker mean?'').
For \hyp{2c}, a subset of \pci items is also asked in ImplicatureX's form, ``Is this interpretation true or false?''.
Multiple-choice options are shuffled on every trial. A subset is also answered without options, to rule out option matching \citep{gong2026think}. Because LLM coding of these open answers did not reach the pre-declared agreement with a human audit, we report them descriptively (\Cref{app:details}).
% TEAM_RULES 1.7/1.7a: LLM labels are never called human; "human" only for the user's audit labels.
Reference labels for these answers are \emph{reference labels by two LLM raters from different model families, adjudicated}: a Claude-family model and Qwen3-32B, with disagreements resolved by a second Claude-family model. We report their inter-rater $\kappa$, and the judge's agreement with them as \emph{consistency}.
Family overlaps are disclosed: Qwen3-32B belongs to the family of the Qwen3 models whose answers it labels; the judge for gpt-oss answers is Qwen3-32B itself, so that agreement is partly self-agreement; the judge for Qwen3 answers, gpt-oss-120b, overlaps with neither rater.
The only human labels are one author's blind audit of \res{gold.v4.n-coding} of these answers and \res{gold.v4.n-a1ctx} speaker-knowledge scenarios, which carries the validity claim (\Cref{app:details}).

\paragraph{Thinking manipulations.}
No thinking (\NT) uses the model's own switch, which leaves the chat template byte-identical apart from the empty thinking block. Two other ways of disabling thinking serve as checks.
Capped budgets stop the thinking block at $B \in \{64, \ldots, 2048\}$ tokens and append Qwen3's own stop phrase \citep{yang2025qwen3}. Because that phrase mentions limited time, a plain cap that appends only the closing tag controls for the time-pressure cue.
Natural thinking (\NAT) is uncapped.
Capping truncates thoughts, so we also stratify eight natural samples per item by their realised length, and we plot every effect against realised rather than nominal length.
Budget forcing beyond the natural stopping point \citep{muennighoff-etal-2025-s1} tests whether more thinking than the model chooses continues the trend.
Capped and length-stratified budgets change only the number of thinking tokens, on fixed weights and a fixed template; the thinking switch and gpt-oss effort levels also change the template or system prompt, so we treat them as mode contrasts and rest dose--response claims on the budget contrasts.
Sampling settings are identical across conditions ($T{=}0.6$, top-$p$ 0.95, top-$k$ 20), so thinking is not confounded with temperature. Generation uses vLLM \citep{kwon2023vllm}.

\paragraph{Interventions and controls.}
\emph{Intent-Seeded Thinking} (\method) places one fixed sentence about speaker intent at the start of the thinking block, or just before it closes. Its controls are a neutral sentence about careful, step-by-step reasoning and a logic sentence about checking what the words strictly entail, both token-matched to the intent seed (26 Qwen3 tokens); a first run used a shorter neutral seed (16 tokens), reported separately and not treated as length-matched.
We compare \method with prompted deliberation on the same weights with thinking off: zero-shot chain-of-thought \citep{kojima2022large}, Gricean instructions and Grice-maxim chain-of-thought \citep{sato2025pragmatic,kim2023pope}, few-shot prompting \citep{ruis2023goldilocks}, an adapted RSA-style chain-of-thought \citep{tsvilodub2025nonliteral}, and self-consistency at matched token cost \citep{wang2023selfconsistency}.
For \hyp{2b}, the critical sentences are preceded by contexts in which the speaker has full or partial knowledge \citep{goodman2013knowledge}.
For \hyp{4}, the load is unrelated background text (512 or 2{,}048 words from one of two genres) placed before the item, followed by an instruction to ignore it.
Each critical item has a comprehension check (an entailment paraphrase) and a meta-pragmatic probe (``Would a speaker who says this normally mean \ldots?''), so a literal answer can be separated from a failure to understand.
\Cref{app:details} gives every prompt verbatim.
Closed-model API calls cost about \$105 in total.

\paragraph{Statistics.}
% Source of truth: notes/STATS_PLAN.md (estimands, families, per-table conventions).
Each condition is run with three decoding seeds. Tables report the mean $\pm$ standard deviation over seeds of the item-averaged rate. Intervals in the text and figures are 95\% cluster-bootstrap confidence intervals over items (10{,}000 resamples, paired across conditions).
The pre-registered primary tests were mixed-effects logistic regressions with by-item random effects; as implemented (\Cref{app:stats}), they are logistic regressions with item-clustered standard errors, one per model, with the log thinking budget, the phenomenon class and their interaction as predictors.
Equivalence is tested with two one-sided tests at $\pm3$\,pp, trends over training steps with Spearman's $\rho$ and permutation $p$-values, and alignment with human rates with Spearman's $\rho$.
$p$-values are Holm-corrected within each pre-registered family of models. Secondary analyses are uncorrected and labelled as such.
Every finding is computed on a held-out half of the items; the other half was used only to fix prompts and parsing. Hypotheses, thresholds and exclusion rules were fixed before the main runs (\Cref{app:stats}).


==> sections/A_floats.tex <==
\section{Additional Figures and Tables}
\label{app:g-floats}
This part collects the full-width figures and large tables referenced in the sections above.

\begin{figure*}[!tp]
  \centering
  \includegraphics[width=\textwidth]{figA_trace_newest.pdf}
  \caption{Trace probe on the newest generation (Qwen3.5-4B, Qwen3.5-9B, Qwen3.8-27B): pragmatic reading $\rate$ after the first $t$ tokens of the model's own trace, with 95\% bands over items. The early lexical-scale jump in the Qwen3.5 panels is systematic and confined to sampled answers (see text).}
  \label{fig:trace-newest}
\end{figure*}

\begin{figure*}[!tp]
  \centering
  \IfFileExists{figures/figA_trace_newfam.pdf}{\includegraphics[width=\textwidth]{figA_trace_newfam.pdf}}{\figplaceholder{\textwidth}{4cm}}
  \caption{Trace probe on further families (EXAONE-Deep-7.8B, Nemotron-Nano-9B-v2, Phi-4-mini-reasoning, Skywork-OR1-7B, Llama-3.1-Nemotron-Nano-8B): pragmatic reading $\rate$ after the first $t$ tokens of the model's own trace, with 95\% bands over items. The $y$-axis runs from 0 to 100 (0 to 80 in \Cref{fig:trace}). In panel (e) the value at $t=0$ is the model's collapse to one answer under a forced-empty thinking block.}
  \label{fig:trace-newfam}
\end{figure*}

\begin{figure*}[p]
  \centering
  \IfFileExists{figures/fig_hero_heatmap.pdf}{\includegraphics[width=\textwidth]{fig_hero_heatmap.pdf}}{\figplaceholder{\textwidth}{5.2cm}}
  \caption{\textbf{Thinking effect for every item family and model.} Change in pragmatic reading with thinking (pp); vermilion: more literal; blue: more pragmatic; framed: 95\% CI excludes 0; hatched: not run. Values in \Cref{tab:main,tab:frontier}.}
  \label{fig:hero-heatmap}
\end{figure*}

\begin{figure*}[!tp]
  \centering
  \includegraphics[width=\textwidth]{fig_hero_dumbbell.pdf}
  \caption{\textbf{Thinking reduces enrichment of \form{some}, \form{or} or both in most tested models; other inference types move differently.} Change in pragmatic reading with thinking (pp, 95\% CI): vermilion, mean of \form{some} and \form{or}; blue, mean of lexical scales and indirect answers; $\blacklozenge$, three-way choice. Every family: \Cref{fig:hero-heatmap}. Q3.5-35B: Qwen3.5-35B-A3B.}
  \label{fig:hero-full}
\end{figure*}

\begin{figure*}[!tp]
  \centering
  \includegraphics[width=\textwidth]{fig_size_family.pdf}
  \caption{\textbf{The literal shift holds across sizes and families.} Thinking effect on \form{some} and \form{or} (pp, 95\% CI) by model size for Qwen3, Qwen3.5 and R1-Distill-Qwen, with Qwen3.8, MiMo, openPangu and DeepSeek-R1-0528 as single points.}
  \label{fig:size}
\end{figure*}

\begin{table*}[!tp]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{4pt}
  \begin{tabularx}{\textwidth}{@{}l >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X l@{}}
    \toprule
    \textbf{Hyp.} & \textbf{Prediction} & \textbf{Outcome (evidence)} & \textbf{Status} \\
    \midrule
    \hyp{1} effort & Pragmatic reading on generalized implicatures rises with thinking & Falls for \form{some} or \form{or} (CI excluding 0) in \res{derived.main.counted} of \res{derived.main.tested} open models, among them EXAONE-Deep-7.8B, Phi-4-mini-reasoning, every newest-generation model (Qwen3.5 0.8B--9B, Qwen3.8-27B), QwQ-32B, Nemotron-Super-49B, R1-Distill-Llama-70B, every Qwen3 size from 1.7B, gpt-oss-20b, OLMo-3-32B-Think, Phi-4-reasoning(-plus), R1-Distill-Llama-8B, MiMo, Nemotron-Nano, AceReason and Skywork-OR1; rises in Magistral-Small (a shift towards answering \emph{Yes}, \Cref{app:frontier}) Granite-3.3, Llama-3.1-Nemotron-Nano-8B (Yes/No format only; literal in the three-way choice) and openPangu-Embedded-7B-model (Yes/No format only; flat in the three-way choice); no significant change in gpt-oss-120b, OLMo-3-7B-Think, SmolLM3 and openPangu-Embedded-7B-V1.1 (\Cref{tab:main}); GPT-5 falls in two formats (\Cref{app:frontier}) & not supported \\
    \hyp{1} default-and-cancel & Falls under the felicity framings, $\geq$5\,pp in $\geq$2 of 4B/8B/14B & \cellcolor{cOurs!5}Holds for \form{some}/\form{or} per family; the pre-registered IMPPRES aggregate at 14B is flat (\res{e1.qwen3-14b.a3.inf.nat.dR.mean}\,pp), so the aggregate gate criterion failed & partly supported \\
    \hyp{1b} capability crossover & Negative at small sizes, positive at $\geq$32B on $\geq$2 families, reproduced in a same-recipe pair & Qwen3-32B negative on \form{some}/\form{or}; OLMo-3-Think 7B null and 32B positive on IMPPRES but negative on \form{some}; no family flips sign within a pair on $\geq$2 families & not supported \\
    \hyp{2} split & \pcis improve while \gcis fall; $\geq$3 \pci sets improve or stay flat & \cellcolor{cOurs!15}Accuracy rises on Fig-QA and PUB at every Qwen3 size from 4B to 32B (8B: +\res{e1xt.qwen3-8b.b3.mc.nat.dacc.mean} and +\res{e1xt.qwen3-8b.b4.mc.nat.dacc.mean}\,pp), on Circa and NOPE in 14 models with no decrease (\Cref{tab:breadth}), and on presupposition and LUDWIG in Qwen3-8B; the budget $\times$ class interaction is significant in Qwen3-4B, 8B and 14B (\Cref{app:stats}) & supported \\
    \hyp{2b} speaker knowledge & Default-and-cancel: thinking lowers $\rate$ in both knowledge conditions; effort/capability: thinking widens the gap & \cellcolor{cCmpA!13}Knowledge sensitivity $\approx$0 in Qwen3 and OLMo; in gpt-oss-120b it shrinks with effort (\res{a1ctx.gpt-oss-120b.a1ctx-fel.fel.low.ksi.mean} $\rightarrow$ \res{a1ctx.gpt-oss-120b.a1ctx-fel.fel.high.ksi.mean}\,pp) & default-and-cancel supported (one model) \\
    \hyp{2c} framing $\times$ class & Truth framing denies implicatures of both classes; meaning framing lets \pcis improve & the interpretation-truth arm was not run & not tested \\
    \bottomrule
  \end{tabularx}
  \caption{Outcome of every pre-registered prediction (held-out split). ``Not tested'' marks predictions whose arm was not run.}
  \label{tab:prereg}
\end{table*}

\begin{table*}[!tp]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \begin{tabularx}{\textwidth}{@{}l >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X l@{}}
    \toprule
    \textbf{Hyp.} & \textbf{Prediction} & \textbf{Outcome (evidence)} & \textbf{Status} \\
    \midrule
    \hyp{3} training origin & The literal shift appears at \rlvr, not SFT; grows with RL steps & Tülu-3: at DPO, before \rlvr; OLMo-3: at thinking SFT, RL-Zero flat, and the thinking cost shrinks over RL steps (\Cref{tab:stages}) & mixed \\
    \hyp{4} load & A load lowers $\rate$ without thinking & \cellcolor{cCmpA!5}With 2{,}048 words of unrelated preceding text and thinking off, $\rate$ on logical words moves from \res{e4.qwen3-8b.a3.L0.off.R.mean} to \res{e4.qwen3-8b.a3.Lx2048.off.R.mean}\% in Qwen3-8B but from \res{e4.qwen3-14b.a3.L0.off.R.mean} to \res{e4.qwen3-14b.a3.Lx2048.off.R.mean}\% in Qwen3-14B; no consistent direction & not supported \\
    \hyp{5} human ordering & $\rho \geq 0.3$ with human rates per scale & not run & not tested \\
    \hyp{6} restorable & \method restores $\geq$50\% of the shift; a length-matched neutral seed does not & \cellcolor{cCmpA!4}With 26-token seeds, the intent seed recovers \res{e10.qwen3-8b.a3-quant.inf.sint.R.mean}\% of a \res{e10.qwen3-8b.a3-quant.inf.off.R.mean}\% no-thinking reading on \form{some} in Qwen3-8B (\NAT: \res{e10.qwen3-8b.a3-quant.inf.nat.R.mean}\%); neutral and logic seeds recover little or none (\Cref{tab:ist}) & partly met: specific to intent, below 50\% \\
    \hyp{7} locus & The literal preference appears inside the trace, after a marker & \cellcolor{cOurs!19}Truncating the model's own trace: the pragmatic reading of \form{some} first rises (Qwen3-8B, +\res{e7.qwen3-8b.a3-quant.inf.p0128.dR.mean}\,pp after 128 tokens) and falls below the no-thinking level later in the trace (\Cref{fig:trace}); literalness markers such as \form{technically} precede the change in only \res{e7f.qwen3-8b.a3f-quant.inf.marker.pre.mean}\% of changing Qwen3-8B traces, and occur as often in traces that do not change (\res{e7f.qwen3-8b.a3f-quant.inf.marker.ctrl_marker.mean}\%) & crossing supported; marker order not supported \\
    \bottomrule
  \end{tabularx}
  \caption*{\Cref{tab:prereg}, continued (part 2 of 3).}
\end{table*}

\begin{table*}[!tp]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \begin{tabularx}{\textwidth}{@{}l >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X l@{}}
    \toprule
    \textbf{Hyp.} & \textbf{Prediction} & \textbf{Outcome (evidence)} & \textbf{Status} \\
    \midrule
    Scenario validity & Humans find \form{some} misleading only under full access ($\geq$80\%) & \cellcolor{cCmpA!15}\res{gold.v4.a1ctx-acc.mean}\% of \res{gold.v4.n-a1ctx} (one author, blind) & met \\
    Open-answer coding & LLM reference rater agrees with the human audit (lower bound of $\kappa \geq 0.40$) & \cellcolor{cCmpA!2}best rater $\kappa$ = \res{gold.v4.kappa-human-a.mean} [\res{gold.v4.kappa-human-a.lo}, \res{gold.v4.kappa-human-a.hi}]; open answers reported descriptively & not met \\
    Bott--Noveck items & Category sentences move with thinking & Near the literal ceiling in every format and condition for Qwen3 4B--32B; only binary felicity at 14B moves & floor set \\
    \bottomrule
  \end{tabularx}
  \caption*{\Cref{tab:prereg}, continued (part 3 of 3).}
\end{table*}

\input{tables/tab_frontier}

\input{tables/tab_frontier_format}

\input{tables/tab_fullsets}

\input{tables/tab_ist}

\input{tables/tab_main}

\input{tables/tab_phen}



==> sections/A_prompts.tex <==
% GENERATED by tools/make_app_v2.py from exp/results/PROMPTS/verbatim.json
\section{Verbatim Prompts}
\label{app:prompts}
Each block shows one fully rendered prompt per format or arm (user turn and, where the arm adds one, the assistant prefix), for one example item.
\paragraph{Yes no inference.} Yes/No inference format (felicity framing), forced-choice letters; the arm tail is appended after the user turn.
\begin{footnotesize}
\begin{verbatim}
A speaker says: "Some teenagers criticize Guy."
Second statement: "Not all teenagers criticize
  Guy."

Would you conclude that the speaker believes the
  second statement is true? Answer Yes or No.

Options:
A. Yes
B. No

Respond with only the letter of the best answer.
\end{verbatim}
\end{footnotesize}
\paragraph{Three way choice.} polarity-free three-way format (NLI): the second statement follows / may be true or false / must be false
\begin{footnotesize}
\begin{verbatim}
First sentence: Some teenagers criticize Guy.
Second sentence: Not all teenagers criticize Guy.

Assume the first sentence is true. Does the second
  sentence follow?

Options:
A. Yes, the second sentence must be true if the
  first is true.
B. Not necessarily: the second sentence may be
  true or false.
C. No, the second sentence must be false if the
  first is true.

Respond with only the letter of the best answer.
\end{verbatim}
\end{footnotesize}
\paragraph{Flipped question.} polarity-flipped felicity question (yes-bias probe): literal answer Yes, pragmatic answer No
\begin{footnotesize}
\begin{verbatim}
A speaker says: "Some guys were cooking."
Second statement: "Not all guys were cooking."

After the speaker's statement, is it still left
  open whether the second statement is true?
  Answer Yes or No.

Options:
A. Yes
B. No

Respond with only the letter of the best answer.
\end{verbatim}
\end{footnotesize}
\paragraph{Circa multiple choice.} multiple-choice format with the dataset's own options
\begin{footnotesize}
\begin{verbatim}
Context: Y has just told X that he/she is
  considering switching his/her job.
X asks: "Do you want a new challenge?"
Y answers: "I've been so bored t work."

What does Y's answer mean?

Options:
A. Yes
B. No
C. Neither yes nor no (in the middle)

Respond with only the letter of the best answer.
\end{verbatim}
\end{footnotesize}
\paragraph{Pub multiple choice.} multiple-choice format with the dataset's own options
\begin{footnotesize}
\begin{verbatim}
Context: Y has just travelled from a different
  city to meet X.
X: Do you want to catch a Christmas movie later?
Y: I hope it is funny.

Choose the best option.

Options:
A. Yes
B. No
C. Yes, subject to some conditions
D. In the middle, neither yes nor no
E. Other

Respond with only the letter of the best answer.
\end{verbatim}
\end{footnotesize}
\paragraph{Budget stop phrase.} think\_b<N> (non-plain): the thought is cut at N tokens and this stop phrase is appended before the close tag; shown for N=0 (empty thought)
\begin{footnotesize}
\begin{verbatim}
<|im_start|>user
Sentence: Some elephants are mammals.

Is this sentence a good way to describe the facts?
  Answer Yes or No.

Options:
A. No
B. Yes

Respond with only the letter of the best
  answer.<|im_end|>
<|im_start|>assistant
<think>


Considering the limited time by the user, I have
  to give the solution based on the thinking
  directly now.
</think>


--> 'B. Yes'
\end{verbatim}
\end{footnotesize}
\paragraph{Trace prefix forced close.} think\_b<N>\_plain: the first N thinking tokens of the SAME trace, then the native close tag (no stop phrase)
\begin{footnotesize}
\begin{verbatim}
<|im_start|>user
Sentence: Some elephants are mammals.

Is this sentence a good way to describe the facts?
  Answer Yes or No.

Options:
A. No
B. Yes

Respond with only the letter of the best
  answer.<|im_end|>
<|im_start|>assistant
<think>
Okay, let's see. The question is whether the
  sentence "Some elephants are mammals" is a good
  way to describe the facts. The options are A
  (No) or B (Yes). I need to answer with just the
  letter.

First, I should recall what elephants are
  classified as. Elephants are a type of mammal.
  The scientific classification of elephants is
  under the class Mammalia. So, all elephants are
  mammals. The sentence says "some elephants are
  mammals," which is technically correct because
  it's a subset. But wait, if all elephants are
  mammals, then saying "some" is still true,
  right? Because "some" means at least one. But is
  it a good way to describe the facts? The
  original statement might be considered accurate,
  but maybe it's not the most precise. However,
  the question is about whether it's a good way to
  describe the facts. Since all elephants are
  mammals, the statement is true, but it's not the
  most comprehensive. However, the question is
  asking if it's a good way, not if it's the best.
  So, if the facts are that all elephants are
  mammals, then "some" is still correct.
  Therefore, the answer would be Yes. But wait,
  maybe the answer is No</think>


--> 'B. Yes'
\end{verbatim}
\end{footnotesize}
\paragraph{Nt off.} thinking switched off: empty thought block in the chat template
\begin{footnotesize}
\begin{verbatim}
<|im_start|>user
Sentence: Some elephants are mammals.

Is this sentence a good way to describe the facts?
  Answer Yes or No.

Options:
A. No
B. Yes

Respond with only the letter of the best
  answer.<|im_end|>
<|im_start|>assistant
<think>

</think>


--> 'B. Yes'
\end{verbatim}
\end{footnotesize}
\paragraph{Forced empty nt.} forced-empty thinking (think\_b0\_plain): the native close tag directly after the opener
\begin{footnotesize}
\begin{verbatim}
<|im_start|>user
A speaker says: "Some teenagers criticize Guy."
Second statement: "Not all teenagers criticize
  Guy."

Would you conclude that the speaker believes the
  second statement is true? Answer Yes or No.

Options:
A. No
B. Yes

Respond with only the letter of the best
  answer.<|im_end|>
<|im_start|>assistant
<think>
</think>


--> 'B'
\end{verbatim}
\end{footnotesize}
\paragraph{Nat.} 
\begin{footnotesize}
\begin{verbatim}
<|im_start|>user
A speaker says: "All teenagers criticize Guy."
Second statement: "Some teenagers criticize Guy."

Would you conclude that the speaker believes the
  second statement is false? Answer Yes or No.

Options:
A. No
B. Yes

Respond with only the letter of the best
  answer.<|im_end|>
<|im_start|>assistant
<think>
Okay, let's try to figure this out. So, the first
  statement is "All teenagers criticize Guy," and
  the second is "Some teenagers criticize Guy."
  The question is whether the speaker believes the
  second statement is false. The options are A
  (No) or B (Yes).

Hmm. Let me think. If someone says "All teenagers
  criticize Guy," does that mean they think "Some
  teenagers criticize Guy" is false? Well, in
  logic, "All" implies that there is at least one.
  So if all teenagers do something, then there
  must be some teenagers doing it. So if the first
  statement is true, then the second statement
  should also be true. Because "some" is a weaker
  statement. So if all teenagers do it, then
  certainly some do it. Therefore, if the speaker
  says "All teenagers criticize Guy," they must
  believe that "Some teenagers criticize Guy" is
  true, not false. Therefore, the speaker does not
  believe the second statement is false. So the
  answer would be No, which is option A. Wait, but
  wait. What if the speaker is lying? Wait, the
  question is about what the speaker believes. If
  the speaker says "All teenagers criticize Guy,"
  then their belief is that all do. But does that
  mean they think that "some" is false? No,
  because "some" is a subset of "all." So if all
  are, then some are. Therefore, the speaker would
  believe that the second statement is true, not
  false. Therefore, the answer is No, so option A.
  But wait, the options are A. No and B. Yes. So
  the question is whether the speaker believes the
  second statement is false. If the speaker
  believes the first statement (all), then they
  would believe the second (some) is true, so they
  don't believe the second is false. So the answer
  is No, so option A.
</think>


--> 'A. No'
\end{verbatim}
\end{footnotesize}


==> sections/A_remedies.tex <==
\section{Remedy Details}
\label{app:remedies}

\subsection{Speaker-Intent Tuning Trains Task-Appropriate Interpretation}
\label{sec:sit}

% METHOD (notes/METHOD_DESIGN.md: v1 seeds and v2 late check failed their pre-declared dev gates; SIT = D-contingency, pre-declared 2026-10-05).

Because early trace prefixes elicit enriched answers that typically vanish by completion, we tested whether a prompt in the thinking channel could preserve them. Both tested interventions, however, fail their pre-declared safety gates on Qwen3-8B development items.

\paragraph{Both tested thinking-channel prompts fail the safety gates.}
On development items for Qwen3-8B, we tested training-free interventions against pre-declared safety gates (\Cref{app:m1dev}).
\begin{itemize}[nosep,leftmargin=*]
  \item \emph{Opening the trace with a sentence about speaker intent} lowers both families. With the route wording, speaker-meaning accuracy falls from \res{m1dev.qwen3-8b.v1.nat.speaker.mean}\% to \res{m1dev.qwen3-8b.v1.route.speaker.mean}\% and literal accuracy from \res{m1dev.qwen3-8b.v1.nat.literal.mean}\% to \res{m1dev.qwen3-8b.v1.route.literal.mean}\%.
  \item \emph{A task-sensitive check before the thinking block closes} (``does the question ask what the words strictly entail, or what the speaker means?'') makes the model more literal still. Speaker-meaning accuracy falls from \res{m1dev.qwen3-8b.v2.nat.speaker.mean}\% to \res{m1dev.qwen3-8b.v2.sitcheck.speaker.mean}\% (\res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.r2w.mean} answers turn wrong, \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.w2r.mean} turn right). A neutral check of the same length leaves it at \res{m1dev.qwen3-8b.v2.neutral.speaker.mean}\%.
\end{itemize}
The task-sensitive check degrades speaker-meaning accuracy more than the same-length neutral check, implicating the prompt's content rather than mere repetition. This motivates training task-appropriate interpretations instead of relying on prompting.

\paragraph{Speaker-Intent Tuning.}
\emph{Speaker-Intent Tuning} (\sit) fine-tunes a model on its own natural-thinking traces, selected so that interpretation is rewarded rather than enrichment.
\begin{itemize}[nosep,leftmargin=*]
  \item \emph{Sampling.} For each training item we sample four traces and keep at most one whose answer matches the original gold label.
  \item \emph{Balance.} Each family gets the same number of traces: speaker meaning, presupposition, and literal-gold items, including logic and arithmetic. The selected traces supervise enriching where the context licenses it and staying literal where the task asks for entailment.
  \item \emph{Difficulty.} Items that the model answers correctly only sometimes fill the quota first, so the signal comes from items where its reading varies.
\end{itemize}
We train LoRA adapters (rank 16; two epochs; settings fixed in advance, final checkpoint only) on Qwen3-8B and on DeepSeek-R1-0528-Qwen3-8B, which shares the base model but has different post-training. The training items come from template families disjoint from both development and test.

\paragraph{Preference variant.} As a fourth and final pre-registered attempt, \sit-DPO trains on pairs of a correct and an incorrect trace for the same item (direct preference optimisation, LoRA, settings fixed in advance), against a control with the pair labels shuffled.

\paragraph{Training settings.} Both trained remedies use LoRA adapters on all attention and MLP projections (rank 16, $\alpha=32$, dropout 0.05), sequences up to 4{,}096 tokens with the loss on thought and answer tokens only, seed 0 and the final checkpoint, all fixed before training. Fine-tuning runs two epochs at learning rate $10^{-4}$ (cosine); preference optimisation runs one epoch at $2\cdot10^{-5}$ with $\beta=0.1$ and the frozen base model as reference. Training items come from template families disjoint from development and test; per family, at most one trace per item is used, with an equal quota per family capped at 1{,}500.

\subsection{Experiments}
\label{sec:sit:results}

\subsubsection{Experimental Settings}
\label{sec:sit:settings}
\textbf{Datasets.} Development items cover the three families of \Cref{sec:sit}; test template families are held out and, because no variant qualified, were never used for any remedy.

\textbf{Baselines.} Each trained variant has a matched control: supervised fine-tuning on the same number of unselected traces, and preference optimisation on the same pairs with shuffled labels. Training-free arms are natural thinking, no thinking, a 512-token budget, a task-aware instruction and the two thinking-channel checks.

\textbf{Metrics.} A variant qualifies for the test set only if it beats natural thinking on the equal-family score and passes one-sided 95\% safety bounds above $-2$\,pp on ImplicatureX cancellation, the true/false framing of the IMPPRES items, FOLIO \citep{han2024folio} and GSM8K \citep{cobbe2021gsm8k}.

\subsubsection{Main Results}
\label{sec:sit:main}
\Cref{tab:dqual} reports the development results of the trained variants. No variant passes the safety gates, and supervised fine-tuning does not beat its own control. In Qwen3-8B, fine-tuning on selected traces scores \res{m1dev.qwen3-8b.d.sit.score.mean}, the same amount of unselected traces \res{m1dev.qwen3-8b.d.control.score.mean}, and natural thinking \res{m1dev.qwen3-8b.d.nat.score.mean}; in DeepSeek-R1-0528-Qwen3-8B the three score \res{m1dev.r1-0528.d.sit.score.mean}, \res{m1dev.r1-0528.d.control.score.mean} and \res{m1dev.r1-0528.d.nat.score.mean}. Tuning shortens the thinking of DeepSeek-R1-0528-Qwen3-8B from \res{m1dev.r1-0528.d.nat.tokfc.mean} to \res{m1dev.r1-0528.d.sit.tokfc.mean} tokens per item, but the unselected control does so as well (\res{m1dev.r1-0528.d.control.tokfc.mean}). Preference optimisation on correct-versus-incorrect pairs edges past its shuffled control, \res{m1dev.qwen3-8b.e.dpo.score.mean} against \res{m1dev.qwen3-8b.e.dposhuf.score.mean} in Qwen3-8B and \res{m1dev.r1-0528.e.dpo.score.mean} against \res{m1dev.r1-0528.e.dposhuf.score.mean} in DeepSeek-R1-0528-Qwen3-8B, where speaker-meaning accuracy rises from \res{m1dev.r1-0528.e.nat.speaker.mean}\% to \res{m1dev.r1-0528.e.dpo.speaker.mean}\%; it still misses the safety gates, so no remedy reached the test set.
\input{tables/tab_dqual}

\textbf{Prompting the thinking backfires.} The task-sensitive late check turns \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.r2w.mean} correct speaker-meaning answers of Qwen3-8B wrong and only \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.w2r.mean} wrong answers right; a neutral check of the same length leaves accuracy at \res{m1dev.qwen3-8b.v2.neutral.speaker.mean}\%. Raising the entailment question is enough to trigger the literal reading that thinking produces on its own.

\subsubsection{Ablation Study}
\label{sec:sit:ablation}
\Cref{tab:ablation} removes one component of \sit at a time on the development items of Qwen3-8B. No training-free intervention passes all safety gates: the late check costs \res{m1dev.qwen3-8b.v2.sitcheck.tr.speaker.r2w.mean} correct speaker-meaning answers, the start-of-thinking seed lowers both families, and even the best training-free arm, the task-aware instruction, misses a gate. Trained on its own traces, the model changes little, and neither component of \sit matters: the full model scores \res{m1dev.qwen3-8b.v3.sit.score.mean}, w/o trace selection \res{m1dev.qwen3-8b.v3.control.score.mean} and w/o family balance \res{m1dev.qwen3-8b.v3.nobal.score.mean}, against \res{m1dev.qwen3-8b.v3.nat.score.mean} for natural thinking.
\input{tables/tab_ablation}

\paragraph{Gate evidence.} \Cref{tab:gates} gives every remedy's per-gate difference and bound, and \Cref{tab:trainsizes} the training sets of the trained remedies.
\input{tables/tab_gates}
\input{tables/tab_trainsizes}

\paragraph{Exploratory inference-time remedies.} After the four pre-registered remedies failed, we froze two exploratory (not pre-registered) inference-time remedies before running them: an early-prefix ensemble that mixes the answer distribution of natural thinking with the answer forced after its first 128 thinking tokens (weight 0.2), and a log-linear blend with the no-thinking answer (weight 0.1). Both apply only to items routed by an input-only rule (the question asks what is meant, implied or intended, the prompt contains \form{some} or \form{or}, and no cancelling phrase); all other items keep the natural-thinking answer. The rule routes \res{m1dev.qwen3-8b.x.routed.mean} of the development items, almost all of them LUDWIG and Circa, and none of the IMPPRES felicity items whose questions do not use those verbs; on the routed items neither remedy changes a single answer, so both score exactly as natural thinking (\Cref{tab:remedies}).

In a second exploratory round, declared before scoring, we swept the weight over $w\in\{0.25,0.5,0.75,1\}$, with $w=1$ answering from the 128-token prefix or from no thinking on routed items, and would have taken the best weight that beats natural thinking within the safety gates to the test set (\Cref{tab:xgrid}). Every weight keeps the gates, but every answer it changes, almost all on LUDWIG, lowers the score: on these context-driven items the completed trace answers better than its early prefix or than no thinking, as the gains of thinking on indirect answers in \Cref{sec:find:split} predict. No weight reached the test set.
\input{tables/tab_xgrid}


==> tables/tab_ablation.tex <==
% GENERATED by tools/make_tab_ablation.py -- do not edit by hand.
\begin{table}[t]
  \centering\small
  \setlength{\tabcolsep}{4pt}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}lrrrr@{}}
    \toprule
    Arm & Speaker & Presup. & Literal & Score \\
    \midrule
    \midrule
    \multicolumn{5}{@{}l}{\emph{Without training}} \\
    Natural thinking & \res{m1dev.qwen3-8b.v2.nat.speaker.mean} & \res{m1dev.qwen3-8b.v2.nat.presup.mean} & \res{m1dev.qwen3-8b.v2.nat.literal.mean} & \res{m1dev.qwen3-8b.v2.nat.score.mean} \\
    Task-aware instruction (user turn) & \res{m1dev.qwen3-8b.v2.taskaware.speaker.mean} & \res{m1dev.qwen3-8b.v2.taskaware.presup.mean} & \res{m1dev.qwen3-8b.v2.taskaware.literal.mean} & \res{m1dev.qwen3-8b.v2.taskaware.score.mean} \\
    Late check: entailment or speaker meaning? & \res{m1dev.qwen3-8b.v2.sitcheck.speaker.mean} & \res{m1dev.qwen3-8b.v2.sitcheck.presup.mean} & \res{m1dev.qwen3-8b.v2.sitcheck.literal.mean} & \res{m1dev.qwen3-8b.v2.sitcheck.score.mean} \\
    Late check: neutral & \res{m1dev.qwen3-8b.v2.neutral.speaker.mean} & \res{m1dev.qwen3-8b.v2.neutral.presup.mean} & \res{m1dev.qwen3-8b.v2.neutral.literal.mean} & \res{m1dev.qwen3-8b.v2.neutral.score.mean} \\
    Start-of-thinking seed (route)$^\ast$ & \res{m1dev.qwen3-8b.v1.route.speaker.mean} & \res{m1dev.qwen3-8b.v1.route.presup.mean} & \res{m1dev.qwen3-8b.v1.route.literal.mean} & \res{m1dev.qwen3-8b.v1.route.score.mean} \\
    \addlinespace[0.5mm]
    \multicolumn{5}{@{}l}{\emph{Trained on own traces}} \\
    \sit w/o trace selection (equal-data control) & \res{m1dev.qwen3-8b.v3.control.speaker.mean} & \res{m1dev.qwen3-8b.v3.control.presup.mean} & \res{m1dev.qwen3-8b.v3.control.literal.mean} & \res{m1dev.qwen3-8b.v3.control.score.mean} \\
    \sit w/o family balance & \res{m1dev.qwen3-8b.v3.nobal.speaker.mean} & \res{m1dev.qwen3-8b.v3.nobal.presup.mean} & \res{m1dev.qwen3-8b.v3.nobal.literal.mean} & \res{m1dev.qwen3-8b.v3.nobal.score.mean} \\
    \midrule
    \ourrow \textbf{\sit (full)} & \res{m1dev.qwen3-8b.v3.sit.speaker.mean} & \res{m1dev.qwen3-8b.v3.sit.presup.mean} & \res{m1dev.qwen3-8b.v3.sit.literal.mean} & \res{m1dev.qwen3-8b.v3.sit.score.mean} \\
    \bottomrule
  \end{tabular}}
  \par\smallskip{\footnotesize $^\ast$From development run~1 (\Cref{tab:m1dev}); all other rows share the same saved thoughts.\par}
  \caption{Ablation of \sit on development items (Qwen3-8B): accuracy (\%) by family; score is the mean of speaker and literal accuracy.}
  \label{tab:ablation}
\end{table}


==> tables/tab_dqual.tex <==
% GENERATED by tools/make_tab_dqual.py -- do not edit by hand.
\begin{table}[t]
  \centering\small
  \setlength{\tabcolsep}{3.5pt}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}lrrrrrc@{}}
    \toprule
    Arm & Speaker & Presup. & Literal & Score & Tokens & Gates \\
    \midrule
    \multicolumn{7}{@{}l}{\textsc{Qwen3-8B}} \\
    Natural thinking & \res{m1dev.qwen3-8b.d.nat.speaker.mean} & \res{m1dev.qwen3-8b.d.nat.presup.mean} & \res{m1dev.qwen3-8b.d.nat.literal.mean} & \res{m1dev.qwen3-8b.d.nat.score.mean} & \res{m1dev.qwen3-8b.d.nat.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.d.nat.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    SFT, unselected traces (control) & \res{m1dev.qwen3-8b.d.control.speaker.mean} & \res{m1dev.qwen3-8b.d.control.presup.mean} & \res{m1dev.qwen3-8b.d.control.literal.mean} & \res{m1dev.qwen3-8b.d.control.score.mean} & \res{m1dev.qwen3-8b.d.control.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.d.control.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \ourrow SFT, selected traces (\sit) & \res{m1dev.qwen3-8b.d.sit.speaker.mean} & \res{m1dev.qwen3-8b.d.sit.presup.mean} & \res{m1dev.qwen3-8b.d.sit.literal.mean} & \res{m1dev.qwen3-8b.d.sit.score.mean} & \res{m1dev.qwen3-8b.d.sit.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.d.sit.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    DPO, shuffled pairs (control) & \res{m1dev.qwen3-8b.e.dposhuf.speaker.mean} & \res{m1dev.qwen3-8b.e.dposhuf.presup.mean} & \res{m1dev.qwen3-8b.e.dposhuf.literal.mean} & \res{m1dev.qwen3-8b.e.dposhuf.score.mean} & \res{m1dev.qwen3-8b.e.dposhuf.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.e.dposhuf.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \ourrow DPO, correct vs.\ incorrect (\sit-DPO) & \res{m1dev.qwen3-8b.e.dpo.speaker.mean} & \res{m1dev.qwen3-8b.e.dpo.presup.mean} & \res{m1dev.qwen3-8b.e.dpo.literal.mean} & \res{m1dev.qwen3-8b.e.dpo.score.mean} & \res{m1dev.qwen3-8b.e.dpo.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.e.dpo.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \addlinespace[0.5mm]\midrule
    \multicolumn{7}{@{}l}{\textsc{DeepSeek-R1-0528-Qwen3-8B}} \\
    Natural thinking & \res{m1dev.r1-0528.d.nat.speaker.mean} & \res{m1dev.r1-0528.d.nat.presup.mean} & \res{m1dev.r1-0528.d.nat.literal.mean} & \res{m1dev.r1-0528.d.nat.score.mean} & \res{m1dev.r1-0528.d.nat.tokfc.mean} & \ifdim\rv{m1dev.r1-0528.d.nat.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    SFT, unselected traces (control) & \res{m1dev.r1-0528.d.control.speaker.mean} & \res{m1dev.r1-0528.d.control.presup.mean} & \res{m1dev.r1-0528.d.control.literal.mean} & \res{m1dev.r1-0528.d.control.score.mean} & \res{m1dev.r1-0528.d.control.tokfc.mean} & \ifdim\rv{m1dev.r1-0528.d.control.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \ourrow SFT, selected traces (\sit) & \res{m1dev.r1-0528.d.sit.speaker.mean} & \res{m1dev.r1-0528.d.sit.presup.mean} & \res{m1dev.r1-0528.d.sit.literal.mean} & \res{m1dev.r1-0528.d.sit.score.mean} & \res{m1dev.r1-0528.d.sit.tokfc.mean} & \ifdim\rv{m1dev.r1-0528.d.sit.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    DPO, shuffled pairs (control) & \res{m1dev.r1-0528.e.dposhuf.speaker.mean} & \res{m1dev.r1-0528.e.dposhuf.presup.mean} & \res{m1dev.r1-0528.e.dposhuf.literal.mean} & \res{m1dev.r1-0528.e.dposhuf.score.mean} & \res{m1dev.r1-0528.e.dposhuf.tokfc.mean} & \ifdim\rv{m1dev.r1-0528.e.dposhuf.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \ourrow DPO, correct vs.\ incorrect (\sit-DPO) & \res{m1dev.r1-0528.e.dpo.speaker.mean} & \res{m1dev.r1-0528.e.dpo.presup.mean} & \res{m1dev.r1-0528.e.dpo.literal.mean} & \res{m1dev.r1-0528.e.dpo.score.mean} & \res{m1dev.r1-0528.e.dpo.tokfc.mean} & \ifdim\rv{m1dev.r1-0528.e.dpo.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \bottomrule
  \end{tabular}}
  \caption{\textbf{Tuning on the model's own traces does not beat its controls.} Development accuracy (\%) by family, score and thinking tokens; \ding{51}: passes all safety gates.}
  \label{tab:dqual}
\end{table}


==> tables/tab_gates.tex <==
% GENERATED by tools/make_app_v2.py
\begin{table*}[t]
  \centering\small
  \begin{tabular}{@{}lllrrrr@{}}
    \toprule
    Remedy & Model & Arm & IX cancel. & IMPPRES true/false & FOLIO & GSM8K \\
    \midrule
    1 Seed (route) & Qwen3-8B & remedy & +0.7 [$-$3.7]\,\ding{55} & $-$3.5 [$-$6.4]\,\ding{55} & $-$6.5 [$-$11.0]\,\ding{55} & $-$16.0 [$-$21.3]\,\ding{55} \\
     &  & control & +0.7 [$-$2.2]\,\ding{55} & +0.1 [$-$0.8] & 0.0 [$-$3.0]\,\ding{55} & $-$1.3 [$-$3.3]\,\ding{55} \\
    \addlinespace[0.5mm]
    2 Late check & Qwen3-8B & remedy & +7.4 [+3.7] & $-$2.8 [$-$4.2]\,\ding{55} & 0.0 [$-$2.5]\,\ding{55} & +0.7 [0.0] \\
     &  & control & 0.0 [0.0] & 0.0 [$-$0.6] & $-$0.5 [$-$2.0]\,\ding{55} & $-$0.7 [$-$2.0]\,\ding{55} \\
    \addlinespace[0.5mm]
    3 SFT & Qwen3-8B & remedy & $-$0.7 [$-$5.1]\,\ding{55} & 0.0 [$-$0.8] & $-$3.0 [$-$5.5]\,\ding{55} & 0.0 [0.0] \\
     &  & control & $-$2.9 [$-$6.6]\,\ding{55} & 0.0 [$-$1.0] & $-$2.5 [$-$5.0]\,\ding{55} & +2.0 [+0.7] \\
     & R1-0528 & remedy & $-$5.9 [$-$10.3]\,\ding{55} & +1.7 [+0.7] & 0.0 [$-$3.5]\,\ding{55} & +2.0 [0.0] \\
     &  & control & $-$5.1 [$-$8.8]\,\ding{55} & +1.4 [+0.3] & +3.0 [0.0] & 0.0 [$-$2.7]\,\ding{55} \\
    \addlinespace[0.5mm]
    4 DPO & Qwen3-8B & remedy & 0.0 [$-$2.9]\,\ding{55} & $-$0.6 [$-$1.6] & $-$1.0 [$-$3.5]\,\ding{55} & +1.3 [0.0] \\
     &  & control & $-$0.7 [$-$4.4]\,\ding{55} & +0.3 [$-$0.4] & $-$2.0 [$-$4.5]\,\ding{55} & +1.3 [0.0] \\
     & R1-0528 & remedy & $-$2.2 [$-$5.9]\,\ding{55} & +0.1 [$-$0.8] & +3.5 [+0.5] & 0.0 [$-$2.7]\,\ding{55} \\
     &  & control & $-$2.2 [$-$5.9]\,\ding{55} & +0.6 [$-$0.3] & +1.5 [$-$1.5] & $-$0.7 [$-$3.3]\,\ding{55} \\
    \addlinespace[0.5mm]
    Task-aware instr. & Qwen3-8B & baseline & $-$0.7 [$-$4.4]\,\ding{55} & +5.5 [+4.0] & $-$1.0 [$-$4.0]\,\ding{55} & +2.0 [+0.7] \\
    \midrule
    \multicolumn{3}{@{}l}{$n$} & 136 & 708 & 200 & 150 \\
    \bottomrule
  \end{tabular}
  \caption{Safety gates of every remedy on development items: paired difference to natural thinking (pp) and, in brackets, its one-sided 95\% lower bound; a gate passes when the bound exceeds $-2$ (\ding{55}: fails). $n$: items per gate.}
  \label{tab:gates}
\end{table*}


==> tables/tab_m1dev.tex <==
% GENERATED by tools/make_tab_m1dev.py -- do not edit by hand.
\begin{table}[t]
  \centering\small
  \setlength{\tabcolsep}{4pt}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{lrrrrrc}
    \toprule
    Arm & Speaker & Presup. & Literal & Score & Tokens & Gates \\
    \midrule
    \multicolumn{7}{l}{\emph{Run 1 (start-of-thinking seeds)}} \\
    No thinking & \res{m1dev.qwen3-8b.v1.nt.speaker.mean} & \res{m1dev.qwen3-8b.v1.nt.presup.mean} & \res{m1dev.qwen3-8b.v1.nt.literal.mean} & \res{m1dev.qwen3-8b.v1.nt.score.mean} & \res{m1dev.qwen3-8b.v1.nt.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.nt.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Natural thinking & \res{m1dev.qwen3-8b.v1.nat.speaker.mean} & \res{m1dev.qwen3-8b.v1.nat.presup.mean} & \res{m1dev.qwen3-8b.v1.nat.literal.mean} & \res{m1dev.qwen3-8b.v1.nat.score.mean} & \res{m1dev.qwen3-8b.v1.nat.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.nat.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Natural, 512-token budget & \res{m1dev.qwen3-8b.v1.nat512.speaker.mean} & \res{m1dev.qwen3-8b.v1.nat512.presup.mean} & \res{m1dev.qwen3-8b.v1.nat512.literal.mean} & \res{m1dev.qwen3-8b.v1.nat512.score.mean} & \res{m1dev.qwen3-8b.v1.nat512.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.nat512.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Task-aware instruction (user turn) & \res{m1dev.qwen3-8b.v1.taskaware.speaker.mean} & \res{m1dev.qwen3-8b.v1.taskaware.presup.mean} & \res{m1dev.qwen3-8b.v1.taskaware.literal.mean} & \res{m1dev.qwen3-8b.v1.taskaware.score.mean} & \res{m1dev.qwen3-8b.v1.taskaware.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.taskaware.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Route text (user turn) & \res{m1dev.qwen3-8b.v1.userroute.speaker.mean} & \res{m1dev.qwen3-8b.v1.userroute.presup.mean} & \res{m1dev.qwen3-8b.v1.userroute.literal.mean} & \res{m1dev.qwen3-8b.v1.userroute.score.mean} & \res{m1dev.qwen3-8b.v1.userroute.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.userroute.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Gricean prefix & \res{m1dev.qwen3-8b.v1.grice.speaker.mean} & \res{m1dev.qwen3-8b.v1.grice.presup.mean} & \res{m1dev.qwen3-8b.v1.grice.literal.mean} & \res{m1dev.qwen3-8b.v1.grice.score.mean} & \res{m1dev.qwen3-8b.v1.grice.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.grice.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Seed: intent & \res{m1dev.qwen3-8b.v1.intent.speaker.mean} & \res{m1dev.qwen3-8b.v1.intent.presup.mean} & \res{m1dev.qwen3-8b.v1.intent.literal.mean} & \res{m1dev.qwen3-8b.v1.intent.score.mean} & \res{m1dev.qwen3-8b.v1.intent.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.intent.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Seed: dual & \res{m1dev.qwen3-8b.v1.dual.speaker.mean} & \res{m1dev.qwen3-8b.v1.dual.presup.mean} & \res{m1dev.qwen3-8b.v1.dual.literal.mean} & \res{m1dev.qwen3-8b.v1.dual.score.mean} & \res{m1dev.qwen3-8b.v1.dual.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.dual.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Seed: route & \res{m1dev.qwen3-8b.v1.route.speaker.mean} & \res{m1dev.qwen3-8b.v1.route.presup.mean} & \res{m1dev.qwen3-8b.v1.route.literal.mean} & \res{m1dev.qwen3-8b.v1.route.score.mean} & \res{m1dev.qwen3-8b.v1.route.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.route.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Seed: task check & \res{m1dev.qwen3-8b.v1.taskcheck.speaker.mean} & \res{m1dev.qwen3-8b.v1.taskcheck.presup.mean} & \res{m1dev.qwen3-8b.v1.taskcheck.literal.mean} & \res{m1dev.qwen3-8b.v1.taskcheck.score.mean} & \res{m1dev.qwen3-8b.v1.taskcheck.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v1.taskcheck.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \multicolumn{7}{l}{\emph{Run 2 (check before the thinking block closes; same stage-1 thoughts)}} \\
    Natural thinking & \res{m1dev.qwen3-8b.v2.nat.speaker.mean} & \res{m1dev.qwen3-8b.v2.nat.presup.mean} & \res{m1dev.qwen3-8b.v2.nat.literal.mean} & \res{m1dev.qwen3-8b.v2.nat.score.mean} & \res{m1dev.qwen3-8b.v2.nat.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v2.nat.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Task-aware instruction (user turn) & \res{m1dev.qwen3-8b.v2.taskaware.speaker.mean} & \res{m1dev.qwen3-8b.v2.taskaware.presup.mean} & \res{m1dev.qwen3-8b.v2.taskaware.literal.mean} & \res{m1dev.qwen3-8b.v2.taskaware.score.mean} & \res{m1dev.qwen3-8b.v2.taskaware.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v2.taskaware.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Late check: entailment or speaker meaning? & \res{m1dev.qwen3-8b.v2.sitcheck.speaker.mean} & \res{m1dev.qwen3-8b.v2.sitcheck.presup.mean} & \res{m1dev.qwen3-8b.v2.sitcheck.literal.mean} & \res{m1dev.qwen3-8b.v2.sitcheck.score.mean} & \res{m1dev.qwen3-8b.v2.sitcheck.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v2.sitcheck.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    Late check: neutral & \res{m1dev.qwen3-8b.v2.neutral.speaker.mean} & \res{m1dev.qwen3-8b.v2.neutral.presup.mean} & \res{m1dev.qwen3-8b.v2.neutral.literal.mean} & \res{m1dev.qwen3-8b.v2.neutral.score.mean} & \res{m1dev.qwen3-8b.v2.neutral.tokfc.mean} & \ifdim\rv{m1dev.qwen3-8b.v2.neutral.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \bottomrule
  \end{tabular}}
  \caption{Training-free interventions on development items (Qwen3-8B). Score: mean of speaker and literal accuracy; tokens per forced-choice item.}
  \label{tab:m1dev}
\end{table}


==> tables/tab_method.tex <==
% PLACEHOLDER skeleton; replaced by tools/make_tab_method.py when SIT test results land.
\begin{table}[t]
  \centering\small
  \setlength{\tabcolsep}{4pt}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{llrrrrr}
    \toprule
    Model & Arm & Speaker & Presup. & Literal & GSM8K & Tokens \\
    \midrule
    Qwen3-8B & Natural thinking & \runcell & \runcell & \runcell & \runcell & \runcell \\
     & Task-aware instruction & \runcell & \runcell & \runcell & \runcell & \runcell \\
     & Equal-data control & \runcell & \runcell & \runcell & \runcell & \runcell \\
     & PragReST-8B (rerun) & \runcell & \runcell & \runcell & \runcell & \runcell \\
    \ourrow  & \textbf{\sit (ours)} & \runcell & \runcell & \runcell & \runcell & \runcell \\
    \addlinespace[0.5mm]\midrule
    DeepSeek-R1-0528-Qwen3-8B & Natural thinking & \runcell & \runcell & \runcell & \runcell & \runcell \\
     & Task-aware instruction & \runcell & \runcell & \runcell & \runcell & \runcell \\
     & Equal-data control & \runcell & \runcell & \runcell & \runcell & \runcell \\
    \ourrow  & \textbf{\sit (ours)} & \runcell & \runcell & \runcell & \runcell & \runcell \\
    \bottomrule
  \end{tabular}}
  \caption{\sit on held-out test families: accuracy (\%) against the original gold and mean generated tokens. \running{cells fill from the running test runs.}}
  \label{tab:method}
\end{table}


==> tables/tab_remedies.tex <==
% GENERATED by tools/make_tab_remedies.py -- do not edit by hand.
\begin{table}[t]
  \centering\small
  \setlength{\tabcolsep}{3pt}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}lllrrrc@{}}
    \toprule
    Remedy & Train & Model & Natural & Remedy & Control & Gates \\
    \midrule
    Seed at start of thinking & none & Qwen3-8B & \res{m1dev.qwen3-8b.v1.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.v1.nat.speaker.mean}} & \res{m1dev.qwen3-8b.v1.route.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.v1.route.speaker.mean}} & \res{m1dev.qwen3-8b.v1.userroute.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.v1.userroute.speaker.mean}} & \ifdim\rv{m1dev.qwen3-8b.v1.route.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \addlinespace[0.5mm]
    Check before thinking ends & none & Qwen3-8B & \res{m1dev.qwen3-8b.v2.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.v2.nat.speaker.mean}} & \res{m1dev.qwen3-8b.v2.sitcheck.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.v2.sitcheck.speaker.mean}} & \res{m1dev.qwen3-8b.v2.neutral.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.v2.neutral.speaker.mean}} & \ifdim\rv{m1dev.qwen3-8b.v2.sitcheck.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \addlinespace[0.5mm]
    SFT on own correct traces & SFT & Qwen3-8B & \res{m1dev.qwen3-8b.d.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.d.nat.speaker.mean}} & \res{m1dev.qwen3-8b.d.sit.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.d.sit.speaker.mean}} & \res{m1dev.qwen3-8b.d.control.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.d.control.speaker.mean}} & \ifdim\rv{m1dev.qwen3-8b.d.sit.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
     &  & R1-0528-Qwen3-8B & \res{m1dev.r1-0528.d.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.d.nat.speaker.mean}} & \res{m1dev.r1-0528.d.sit.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.d.sit.speaker.mean}} & \res{m1dev.r1-0528.d.control.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.d.control.speaker.mean}} & \ifdim\rv{m1dev.r1-0528.d.sit.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \addlinespace[0.5mm]
    DPO, correct vs.\ incorrect & DPO & Qwen3-8B & \res{m1dev.qwen3-8b.e.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.e.nat.speaker.mean}} & \res{m1dev.qwen3-8b.e.dpo.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.e.dpo.speaker.mean}} & \res{m1dev.qwen3-8b.e.dposhuf.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.e.dposhuf.speaker.mean}} & \ifdim\rv{m1dev.qwen3-8b.e.dpo.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
     &  & R1-0528-Qwen3-8B & \res{m1dev.r1-0528.e.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.e.nat.speaker.mean}} & \res{m1dev.r1-0528.e.dpo.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.e.dpo.speaker.mean}} & \res{m1dev.r1-0528.e.dposhuf.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.e.dposhuf.speaker.mean}} & \ifdim\rv{m1dev.r1-0528.e.dpo.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \addlinespace[0.5mm]
    Early-prefix ensemble$^\dagger$ & none & Qwen3-8B & \res{m1dev.qwen3-8b.x.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.x.nat.speaker.mean}} & \res{m1dev.qwen3-8b.x.x1.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.x.x1.speaker.mean}} & \res{m1dev.qwen3-8b.x.x1w0.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.x.x1w0.speaker.mean}} & \ifdim\rv{m1dev.qwen3-8b.x.x1.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
     &  & R1-0528-Qwen3-8B & \res{m1dev.r1-0528.x.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.x.nat.speaker.mean}} & \res{m1dev.r1-0528.x.x1.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.x.x1.speaker.mean}} & \res{m1dev.r1-0528.x.x1w0.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.x.x1w0.speaker.mean}} & \ifdim\rv{m1dev.r1-0528.x.x1.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \addlinespace[0.5mm]
    No-think blend$^\dagger$ & none & Qwen3-8B & \res{m1dev.qwen3-8b.x.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.x.nat.speaker.mean}} & \res{m1dev.qwen3-8b.x.x2.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.x.x2.speaker.mean}} & \res{m1dev.qwen3-8b.x.x2w0.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.qwen3-8b.x.x2w0.speaker.mean}} & \ifdim\rv{m1dev.qwen3-8b.x.x2.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
     &  & R1-0528-Qwen3-8B & \res{m1dev.r1-0528.x.nat.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.x.nat.speaker.mean}} & \res{m1dev.r1-0528.x.x2.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.x.x2.speaker.mean}} & \res{m1dev.r1-0528.x.x2w0.score.mean}\,\textcolor{gray}{\scriptsize \res{m1dev.r1-0528.x.x2w0.speaker.mean}} & \ifdim\rv{m1dev.r1-0528.x.x2.gates.mean}pt>0.5pt \ding{51}\else \ding{55}\fi \\
    \bottomrule
  \end{tabular}}
  \par\smallskip{\footnotesize Controls: same text in the user turn; neutral check; unselected traces; shuffled pairs; weight 0. $^\dagger$Exploratory, not pre-registered. Details: \Cref{app:remedies}.\par}
  \caption{\textbf{No remedy passes its safety gates.} Development score (mean of speaker-meaning and literal accuracy, \%) for natural thinking, the remedy and its control; speaker-meaning accuracy in gray.}
  \label{tab:remedies}
\end{table}


==> tables/tab_sit_setup.tex <==
% Hand-written design table (item counts from exp/data/items/method_test.jsonl, method_gsm_test.jsonl).
\begin{table*}[t]
  \centering\small
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}lll@{}}
    \toprule
    \multicolumn{3}{@{}l}{\emph{Test sets} (items)} \\
    Speaker meaning & \multicolumn{2}{l}{IMPPRES \form{some}/\form{or} felicity (250/242), ImplicatureX recognition (135),} \\
     & \multicolumn{2}{l}{LUDWIG (136), Circa (250), PUB T2/T3/T6 (75 each), Fig-QA (245)} \\
    Presupposition & \multicolumn{2}{l}{NOPE (342), IMPPRES presupposition (300)} \\
    Literal gold & \multicolumn{2}{l}{ImplicatureX cancellation (135), IMPPRES true/false (250/242),} \\
     & \multicolumn{2}{l}{FOLIO (203), GSM8K (500)} \\
    \midrule
    \emph{Arm} & \emph{Training} & \emph{What it controls for} \\
    Natural thinking & none & reference \\
    No thinking; 512-token budget & none & less deliberation \\
    Task-aware instruction (user turn) & none & strongest prompt on development \\
    Equal-data SFT control & LoRA, unselected traces & fine-tuning on own traces \\
    PragReST (our rerun) & published RL & trained competitor \\
    \ourrow \textbf{\sit (ours)} & LoRA, selected traces & trace selection, family balance \\
    \bottomrule
  \end{tabular}
  \caption{\sit evaluation: test sets by family and compared arms, all on the same weights except the trained rows.}
  \label{tab:sit:setup}
\end{table*}


==> tables/tab_trainsizes.tex <==
% GENERATED by tools/make_app_v2.py
\begin{table}[t]
  \centering\small
  \begin{tabular}{@{}llrr@{}}
    \toprule
    Model & Family & Traces & Mixed share \\
    \midrule
    Qwen3-8B & speaker & 1{,}318 & 36.3\% \\
     & literal & 1{,}318 & 14.9\% \\
     & presup & 1{,}318 & 29.8\% \\
    \addlinespace[0.5mm]
    R1-0528-Qwen3-8B & speaker & 1{,}404 & 39.0\% \\
     & literal & 1{,}404 & 14.6\% \\
     & presup & 1{,}404 & 35.3\% \\
    \bottomrule
  \end{tabular}
  \caption{Training sets of the trained remedies: traces per family (equal quota), and the share drawn from items the model answers correctly in only 1--3 of 4 samples.}
  \label{tab:trainsizes}
\end{table}


==> tables/tab_xgrid.tex <==
% GENERATED by tools/make_app_v2.py from selection_dev_X2_*.json
\begin{table}[t]
  \centering\small
  \setlength{\tabcolsep}{3pt}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}llrrrrr@{}}
    \toprule
    Model & Remedy & $w{=}0$ & 0.25 & 0.5 & 0.75 & 1.0 \\
    \midrule
    Qwen3-8B & X1$'$ & 73.04 & 73.04 [0] & 73.00 [4] & 72.79 [43] & 72.72 [44] \\
     & X2$'$ & 73.04 & 73.03 [1] & 73.00 [6] & 72.95 [33] & 72.77 [54] \\
    \addlinespace[0.5mm]
    R1-0528-Qwen3-8B & X1$'$ & 71.06 & 71.06 [0] & 70.95 [7] & 70.66 [39] & 70.58 [55] \\
     & X2$'$ & 71.06 & 71.06 [0] & 71.04 [1] & 70.92 [9] & 70.58 [61] \\
    \bottomrule
  \end{tabular}}
  \caption{Exploratory round 2: development score of the early-prefix ensemble (X1$'$) and the no-thinking blend (X2$'$) over the pre-declared weight grid; answers changed relative to natural thinking in brackets. No weight beats natural thinking, so neither reached the test set.}
  \label{tab:xgrid}
\end{table}

